Measurement of the Electron Neutrino Charged-current Interaction Rate on Water with the T2K ND280 pi-zero Detector

This paper presents a measurement of the charged current interaction rate of the electron neutrino beam component of the beam above $1.5$~GeV using the large fiducial mass of the T2K $\pi^0$ detector. The predominant poriton of the $\nu_e$ flux ($\sim$85 %) at these energies comes from kaon decays. The measured ratio of the observed beam interaction rate to the predicted rate in the detector with water targets filled is 0.89 $\pm$ 0.08 (stat.) $\pm$ 0.11 (sys.), and with the water targets emptied is 0.90 $\pm$ 0.09 (stat.) $\pm$ 0.13 (sys.). The ratio obtained for the interactions on water only from an event subtraction method is 0.87 $\pm$ 0.33 (stat.) $\pm$ 0.21 (sys.). This is the first measurement of the interaction rate of electron neutrinos on water, which is particularly of interest to experiments with water Cherenkov detectors.

==> Makefile <==
TEX = pdflatex
BIB = bibtex
#main file
texfile = P0DNuE
FIGS=$(wildcard figures/*.*)
#all texfiles
SECS=$(wildcard *.tex)

#REVTEX:=$(CURDIR)/revtex4-1/tex/latex/revtex
#REVBST:=$(CURDIR)/revtex4-1/bibtex/bst/revtex

#export TEXINPUTS:=$(CURDIR):$(REVTEX):$(TEXINPUTS)
#export BSTINPUTS:=$(CURDIR):$(REVBST):$(BSTINPUTS)
export TEXINPUTS:=$(CURDIR):$(TEXINPUTS)
export BSTINPUTS:=$(CURDIR):$(BSTINPUTS)


.PHONY: pdf
.PHONY: clean

all: pdf

pdf: $(texfile).pdf

$(texfile).pdf : $(SECS) $(FIGS) $(texfile).bib
	$(TEX) --shell-escape --synctex=1 $(texfile)
	$(BIB) $(texfile)
	$(TEX) --shell-escape --synctex=1 $(texfile)
	$(TEX) --shell-escape --synctex=1 $(texfile)

clean:
	@ls $(texfile).* | grep -v '.tex\|.bib' | xargs -I {} rm {}

revtex: 
	mktexlsr $(PWD)/revtex4-1

